Certified MaxSAT Preprocessing

Building on the progress in Boolean satisfiability (SAT) solving over the last decades, maximum satisfiability (MaxSAT) has become a viable approach for solving NP-hard optimization problems, but ensuring correctness of MaxSAT solvers has remained an important concern. For SAT, this is largely a solved problem thanks to the use of proof logging, meaning that solvers emit machine-verifiable proofs of (un)satisfiability to certify correctness. However, for MaxSAT, proof logging solvers have started being developed only very recently. Moreover, these nascent efforts have only targeted the core solving process, ignoring the preprocessing phase where input problem instances can be substantially reformulated before being passed on to the solver proper. In this work, we demonstrate how pseudo-Boolean proof logging can be used to certify the correctness of a wide range of modern MaxSAT preprocessing techniques. By combining and extending the VeriPB and CakePB tools, we provide formally verified, end-to-end proof checking that the input and preprocessed output MaxSAT problem instances have the same optimal value. An extensive evaluation on applied MaxSAT benchmarks shows that our approach is feasible in practice.

==> removed.tex <==

%Moved commented stuff away from other documents to here


\iffalse
\subsection{Proof logging in practice}
\TODO{moved from sec 3 where this was shortened. }
\label{sec:preprocessing-techniques}

In the following, we detail proof logging for selected preprocessing techniques as concrete examples of how proof logging for preprocessing looks like in practice.
A complete overview of proof logging for all techniques of MaxPRE~2~\cite{DBLP:conf/sat/KorhonenBSJ17,IBJ22ClauseRedundancy}
(including removal of tautologies and duplicate clauses, unit propagation, bounded variable elimination~\cite{DBLP:conf/sat/SubbarayanP04a,EB05EffectivePreprocessing},
bounded variable addition~\cite{MHB12AutomatedReencoding}, blocked clause elimination~\cite{DBLP:conf/tacas/JarvisaloBH10}, subsumption elimination,
self-subsuming resolution~\cite{DBLP:conf/cp/OstrowskiGMS02,EB05EffectivePreprocessing},
\TODO{SIE}, failed literal elimination~\cite{DBLP:conf/aaai/ZabihM88,Freeman1995ImprovementsPropositionalSatisfiability,DBLP:journals/endm/Berre01},
equivalent literal substitution~\cite{DBLP:conf/aaai/Li00,DBLP:journals/tsmc/Brafman04,DBLP:journals/amai/Gelder05},
TrimMaxSAT~\cite{DBLP:conf/vmcai/PaxianRB21}, \TODO{group detection~\cite{something}}, (group)-subsumed label elimination~\cite{DBLP:conf/ecai/BergSJ16,DBLP:conf/sat/KorhonenBSJ17},
intrinsic at-most-ones~\cite{DBLP:journals/jsat/IgnatievMM19,IBJ22ClauseRedundancy},
binary core removal~\cite{DBLP:conf/focs/Gimpel64,DBLP:conf/sat/KorhonenBSJ17}, label matching~\cite{DBLP:conf/sat/KorhonenBSJ17},
and hardening~\cite{DBLP:conf/sat/MorgadoHM12,DBLP:conf/cp/AnsoteguiBGL12,IBJ22ClauseRedundancy}) is given in Appendix~\ref{apx:prepro}.

\subsubsection{Bounded Variable Elimination (BVE)~\cite{DBLP:conf/sat/SubbarayanP04a,EB05EffectivePreprocessing}.}
Given (non-objective) variable $x$ and CNF-formula $\formula$, BVE eliminates $x$ from the formula as follows.
Consider two sets of clauses of $\formula$: $\mathcal{C}_{x}=\{C\mid x\in C\}$ and $\mathcal{D}_{\olnot{x}}=\{D\mid \olnot{x}\in D\}$.
BVE replaces all clauses in $\mathcal{C}_x$ and $\mathcal{D}_{\olnot{x}}$ with non-tautological clauses in $\mathcal{C}_{x}\otimes \mathcal{D}_{\olnot{x}} = \{C_x\otimes D_{\olnot{x}}\mid C_x\in \mathcal{C}_{x}, D_{\olnot{x}}\in \mathcal{D}_{\olnot{x}}\}$, where $(C\lor x) \otimes (D\lor \olnot{x}) = C\lor D$.

The proof is logged as follows.
First, introduce all non-tautological clauses in $\mathcal{C}_{x}\otimes \mathcal{D}_{\olnot{x}}$ and move these clauses immediately to the set of core constraints.
Each clause $C_x\otimes D_{\olnot{x}}$ is derived as a sum of existing constraints $C_x$ and $D_{\olnot{x}}$.
To remove clauses in $\mathcal{C}_x$ and $\mathcal{D}_{\olnot{x}}$, checked deletion is used, with witnesses $\omega=\{x\rightarrow 1\}$ and $\omega=\{x\rightarrow 0\}$, respectively.
\TODO{(Redundance based strengthening with a single literal as a witness corresponds to RAT.)}

\subsubsection{TrimMaxSAT~\cite{DBLP:conf/vmcai/PaxianRB21}.}
Given a set $T$ of literals, TrimMaxSAT algorithm finds a subset $N\subseteq T$ of them such that for each $l\in N$, $\formula \ent \{\olnot{l}\}$.
Given such a set $N$ computed by TrimMaxSAT, each literal $\olnot{l}$ is fixed, i.e., the following simplifications are applied:
each clause $C\lor l$ is replaced with $C$, and each clause $C\lor \olnot{l}$ is removed from the instance.


To find set $N$, TrimMaxSAT algorithm initializes $N=T$ and iterively updates $N$ by heuristically looking for solutions and removing literals assigned to $1$ by those solutions.
A(n incremental) SAT solver with assumption interface~\cite{DBLP:journals/entcs/EenS03,DBLP:conf/sat/AudemardLS13} is used.
When such a SAT solver---initialized with $\formula$---is invoked with a set of literals $A$ as assumptions,
it either returns a solution $\tau$ to $\formula$ with $\tau(l)=1$ for each $l\in A$ (SAT),
or determines that such a solution does not exist (UNSAT).
TrimMaxSAT initializes the SAT solver with the hard clauses of the instance at hand, and introduces some additional clauses to the SAT solver. 
More precisely, in each iteration of TrimMaxSAT, the current set of literals $N$ is divided to $m$ subsets.
For each subset (i.e. clause) $S_i$, a clause $S_i\lor s_i$ is introduced to the formula of SAT solver, where $s_i$ is a fresh variable.
Then a SAT solver is invoked with assumptions $\olnot{s}_i$ for each $i$.


If the SAT solver returns SAT, each literal in $N$ assigned to $1$ by the solution is removed from $N$.
If the SAT solver returns UNSAT for a value $m > 1$, the value of $m$ is decreased.
The algorithm finishes when $m=1$ and the SAT solver returns UNSAT, or when $N=\emptyset$.
\TODO{(Notice that if $m=1$ and SAT solver returns SAT, after each $l\in N$ will be included in the solution returned by the SAT solver, and
after $N$ is updated, $N=\emptyset$.)}
In the former case, $N$ contains literals that are not satisfied by any feasible solution to $\formula$.
Then each $l\in N$ is `fixed' to $0$.
For an intuitive explanation of TrimMaxSATs correctness, note that when $m=1$ the assumptions $\olnot{s}_i$ enforce at least one of the literal  $N$ to $1$,
if the result is UNSAT we can conclude every solution assigns all literals in $N$ to $0$.

When TrimMaxSAT algorithm is iterated, the proof is logged as follows.
Each SAT solver call produces a proof where each learnt clause is introduced as a RUP clause (these clauses are \emph{not} moved to the core set)\cite{something}.
When TrimMaxSAT algorithm has found the final (non-empty) set of literals $N$, an additional SAT solver call is performed for each literal $l\in N$.
The SAT solver is called under assumption $l$, which results in UNSAT.
After this additional SAT solver call, $\{\olnot{l}\}$ is guaranteed to be RUP clause wrt the current formula.
Then, each $\{\olnot{l}\}$ is introduced as a RUP clause to the instance and this clause is moved to the core set.

In the end of TrimMaxSAT technique, when SAT solver will not be used for any new calls, we do the following.
All clauses learnt by SAT solver are removed from the proof.
(As they are not in derived set, they can be removed without further considerations.)
Then the simplifications that follow from `fixing' each literal $\olnot{l}$ are applied.
To replace each $C\lor l$ with $C$, we introduce $C$ as a sum of constraints $C\lor l$ and $\{\olnot{l}\}$ and remove constraint $C\lor l$.
Then we remove each constraint $C\lor \olnot{l}$ from the instance and finally, we remove the constraint $\{\olnot{l}\}$ with witness $\omega=\olnot{l}$.
The `fixing' of literals is done after finishing with SAT solver, because it may remove clauses from the core set,
\TODO{and checked deletion---in principle---requires that the derived set is empty (some relaxation for this rule can be used though, see~\cite{something}).}.


\subsubsection{Label matching~\cite{DBLP:conf/sat/KorhonenBSJ17}.}
Assume that
(i) $\formula$ contains clauses $C\lor b_C$ and $D\lor b_D$
(ii) $b_C$ and $b_D$ are objective literals with the same coefficient in $\obj$,
(iii) Variables $b_C$ and $b_D$ do not appear (in either polarity) in other clauses of $\formula$, (iv) $C\lor D$ is a tautology.
Label matching replaces $b_C$ and $b_D$ with a fresh variable $b_{CD}$ (i.e., remove clauses $C\lor b_C$ and $D\lor b_D$, introduce $C\lor b_{CD}$, $D\lor b_{CD}$ instead) and adds $-wb_C-wb_D+wb_{CD}$ to the objective function.

As $C \lor D$ is a tautology we can w.l.o.g. assume that $\bar{x}\in C$ and  $x \in D$ for some variable $x$.
Label matching is logged in the following way.
First, we introduce clause $\{\olnot{b}_C, \olnot{b}_D\}$ with witness $\omega=\{b_C\rightarrow x, b_D\rightarrow \olnot{x}\}$.
Indeed, even though there may be (\TODO{or are?}) some solutions that do not satisfy this clause, every optimal solution sets either $b_C=0$ or $b_D=0$.

The next step is to introduce a new variable $b_{CD}$, with encoding $b_{CD} = b_C + b_D$.
The clause $\{b_C, b_D\}$ introduced first makes possible that the equality holds even though the variables are binary.

Then, we update the objective function by adding $-wb_C-wb_D+wb_{CD}$.
The encoding of $b_{CD}$ makes this step correct.
Next step is to introduce clauses $C\lor b_{CD}$ and $D\lor b_{CD}$ to replace $C\lor b_C$ and $D\lor b_D$.
The new clauses are RUP; falsifying $C\lor b_{CD}$ will unit propagate $b_{CD}=0$ which means that the clause $C\lor b_C$ is falsified (and similarly for $D\lor b_{CD}$).
To delete $C\lor b_C$ and $D\lor b_D$ we use witness $\omega=\{b_C\rightarrow \olnot{x}, b_D\rightarrow x\}$.

Finally, we delete the constraints used to define $b_{CD} = b_C + b_D$ and clause $\{\olnot{b}_C, \olnot{b}_D\}$.

\subsubsection{Binary core removal~\cite{DBLP:conf/focs/Gimpel64,DBLP:conf/sat/KorhonenBSJ17} \TODO{say something like ``MaxSAT equivalent of Gimpel's reduction rule''?}.}
Assume the following three things: (i) $F$ contains a clause $\{b_C, b_D\}$ for two objective literals $b_C$ and $b_D$, (ii) $b_C$ and $b_D$ have the same coefficient $w$ in $O$, and (iii) the negations $b_C$ and $b_D$ do not appear in any clauses of $F$.
Assume additionally that $b_C$ and $b_D$ do not appear together in other clauses than in the core $\{b_C, b_D\}$ and that both appear in at least one other clause of $F$.
Binary core removal replaces all clauses where $b_C$ or $b_D$ appear with non-tautological clauses in $\{ C\cup D\cup \{b_{CD}\}\setminus\{b_C, b_D\}  \mid b_C\in C, b_D\in D\}$, where $b_{CD}$ is a fresh variable. Additionally, the objective function is modified by adding $-w b_C -w b_D +wb_{CD}+w$.

Our proof for binary core removal comes from seeing it as subsequent applications of two other preprocessing techniques, intrinsic at-most-ones and (bounded) variable elimination.

\TODO{The first step of our proof for binary core removal is thus to apply so-called intrinsic at-most-ones technique~\cite{DBLP:journals/jsat/IgnatievMM19,IBJ22ClauseRedundancy} for variables $b_C$ and $b_D$.}
Given a set $L$ of objective literals such that $\sum_{b\in L}b\ge |L|-1$, this technique introduces a new clause $\{\olnot{b}\mid b\in L\}\cup\{b^L\}$ (where $b^L$ is a fresh variable) and additionally, $\sum_{b\in L} -w^Lb+w^Lb^L+|L-1|w^L$ is added to the objective function, where $w^L=\min (\{c^{b}\mid b\in L\})$.
Proof logging for intrinsic at-most-ones has been previously studied in~\cite{BBNOV23CertifiedCoreGuided}.
Thus we do not detail the proof here.
After applying intrinsic-at-most ones as a substep, $-wb_C-wb_D+wb_{CD}+w$ has been added to the objective and clause $\{\olnot{b}_C, \olnot{b}_D, b_{CD}\}$ has been introduced to the instance as a new clause.
Notice that now $b_C$ and $b_D$ are no longer objective variables, which enables to use variable elimination on them.

The second step is to apply variable elimination on variable $b_C$.
Literal $b_C$ appears in clause $\{b_C, b_D\}$ and a set of clauses of form $C_i\lor b_C$.
Literal $\olnot{b}_C$ appears only in clause $\{\olnot{b}_C, \olnot{b}_D, b_{CD}\}$ (the clause introduced during the at-most-ones step).
Variable elimination on $b_C$ yields a set of clauses
$C_i\lor b_D \lor b_{CD}$. The original clauses are all removed.

The final step is to apply bounded variable elimination on variable $b_D$.
At this point, the literal $b_D$ appears in a set of clauses of form $D_i\lor b_D$ and literal $\olnot{b}_D$ appears in clauses $C_i\lor \olnot{b}_D \lor b_{CD}$.
Bounded variable elimination on $b_D$ thus yields clauses $C_i\lor D_i\lor b_{CD}$, and the proof is completed.

\fi




\iffalse
Preprocessing (under \emph{equioptimality}) applies a series of preprocessing rules to convert a MaxSAT instance $\instance$ into an \emph{equioptimal} instance $\instance'$, i.e., into an instance $\instance'$ such that $\opt(\instance)=\opt(\instance')$.
In the context of MaxSAT, the preprocessing r do three types of modifications to the instance:

\begin{itemize}
\item[(1)] Introduce a new clause $C$, that is redundant wrt MaxSAT instance $\instance$.
\item[(2)] Remove a redundant clause $C \in \formula$ from the instance.
\item[(3)] Change the objective function $\obj$.
\end{itemize}

The following example illustrates how preprocessing could modify a MaxSAT instance.
\begin{example}\label{ex:prepro} Consider a MaxSAT instance $\instance$ with clauses $\{x, \olnot{b}_1\}$, $\{\olnot{x}, \olnot{b}_1\}$, and $\{x, b_1, \olnot{b}_2\}$, and objective $\obj \equiv 2\olnot{b}_1+\olnot{b}_2$. The following steps provide an example of how $\instance$ could be preprocessed.

\begin{itemize}
\item[(i)] Introduce new clause $\{\olnot{b}_1\}$; it is derived from clauses $\{x, \olnot{b}_1\}$, $\{\olnot{x}, \olnot{b}_1\}$.
\item[(ii)] Change the bjective function to $\obj \equiv\olnot{b}_1+2$; follo ws from the unit clause $\{\olnot{b}_1\}$.
\item[(iii)] Remove all clauses with $\olnot{b}_1$ in them and remove all occurrences of $b_1$ from remaining clauses; follows from the unit clause $\{\olnot{b}_1\}$. After this, the remaining instance is
clause $\{x, \olnot{b}_2\}$ with objective $O\equiv \olnot{b}_2 + 2$
\item[(iv)] Introduce unit clause $\{x\}$ and do similar simplifications as in step (iii); this is sound as variable $x$ only occurs in clause $\{x, \olnot{b}_2\}$. After this, there are no clauses remaining and the objective is $\obj \equiv \olnot{b}_2 + 2$.
\item[(v)] Introduce unit clause $\{b_2\}$, update the objective function to $\obj \equiv 2$; $\olnot{b}_2$ does not occur in any clauses and because of the objective, we prefer $b_2=1$ to $b_2=0$.
\end{itemize}

\end{example}

There are two types of preprocessing techniques for MaxSAT which we will consider in this paper:
(1) liftings of SAT-based preprocessing techniques to MaxSAT
and (2) MaxSAT-specific preprocessing techniques.
MaxSAT-specific techniques differ from SAT-based techniques in that they apply objective function in the reasoning.
Each preprocessing techniques may perform one or more of the three types of modifications.

\TODO{This is probably too lengthy...}
To give some concreteness to what the preprocessing techniques actually do, we now shortly describe each MaxSAT preprocessing technique for which we develop proof logging in this work (the list containst the proof logging techniques implemented in a state-of-the-art MaxSAT preprocessor \maxpre~2~\cite{DBLP:conf/sat/KorhonenBSJ17,IBJ22ClauseRedundancy}).
We consider SAT-based and MaxSAT-specific techniques separately.
The SAT-based techniques are the following.
\begin{itemize}
\item \textbf{Removing tautologies}: if the instance has clause $C\lor x \lor \olnot{x}$, $C$ is removed.
\item \textbf{Removing duplicate clauses}: if the instance has clauses $C$ and $D$ such that $C=D$, $D$ is removed.
\item \textbf{Unit Propagation}: if the instance has a unit clause $\{l\}$, unit propagation removes each clause in $\{C\mid l\in C\}$ and replaces each clause  $C_{\olnot{l}}\in \{C\mid \olnot{l}\in C\}$ with $C_{\olnot{l}}\setminus \{\olnot{l}\}$.
\item \textbf{Bounded Variable Elimination}~\cite{DBLP:conf/sat/SubbarayanP04a,EB05EffectivePreprocessing}: given a variable $x$ and a CNF-formula $\formula$, bounded variable elimination replaces all clauses in $\mathcal{C}_{x}=\{C\mid x\in C\}$ and $\mathcal{D}_{\olnot{x}}=\{C\mid \olnot{x}\in C\}$ with clauses in $\mathcal{C}_{x}\otimes \mathcal{D}_{\olnot{x}} = \{C_x\otimes D_{\olnot{x}}\mid C\in \mathcal{C}_{x}, D_{\olnot{x}}\in \mathcal{D}_{\olnot{x}}\}$, where $(C\lor x) \otimes (D\lor \olnot{x}) = C\lor D$.
\item \textbf{Bounded Variable Addition}~\cite{MHB12AutomatedReencoding}: in a complementary manner to bounded variable elimination, bounded variable addition introduces a new variable $x$ and replaces a set of clauses with another.
\item \textbf{Blocked Clause Elimination}~\cite{DBLP:conf/tacas/JarvisaloBH10}: given a clause $C$ and a literal $l\in C$, if each clause $C_{\olnot{l}} \in \{C\mid \olnot{l}\in C\}$ has a literal $l'\in C_{\olnot{l}}$ such that $\olnot{l'}\in C$, blocked clause elimination removes $C$.
\item \textbf{Subsumption Elimination}: if the instance has clauses $C$ and $D$ such that $C\subseteq D$, $D$ is removed.
\item \textbf{Self-Subsuming Resolution}~\cite{DBLP:conf/cp/OstrowskiGMS02,EB05EffectivePreprocessing}: if the instance has clauses $C\lor x$ and $D\lor \olnot{x}$ such that $C\subseteq D$, self-subsuming resolution replaces $D\lor \olnot{x}$ with $D$.
\item \textbf{\TODO{SIE}}: if the instance has two literals $x$ and $y$ such that $x\in C_{\olnot{y}}$ for each $C_{\olnot{y}}\in\{C\mid \olnot{y}\in C\}$ and $y\in C_{\olnot{x}}$ for each $C_{\olnot{c}}\in\{C\mid \olnot{x}\in C\}$, introduce unit clauses $\{x\}$ and $\{y\}$ and apply unit propagation.
\item \textbf{Failed Literal Elimination}~\cite{DBLP:conf/aaai/ZabihM88,Freeman1995ImprovementsPropositionalSatisfiability,DBLP:journals/endm/Berre01}. In the following, we write $x \up y$ if introducing unit clause $\{x\}$ to $F$ and applying unit propagation steps until the fixpoint allows to infer unit clause $\{y\}$ and we write $x\up \confl$ if introducing $\{x\}$ to $F$ and applying unit propagation until the fixpoint infers conflict. Given that $x\up \confl$, failed literal elimination introduces unit clause $\{\olnot{x}\}$ to the instance and applies unit propagation rule to remove variable $x$.
\item \TODO{\textbf{``Implied Literal Detection''?}}: if $x\up y$ and $\olnot{x}\up y$, \TODO{implied literal detection} introduces unit clause $\{y\}$ and applies unit propagation rule to remove variable $y$.
\item \textbf{Equivalent Literal Substitution}:~\cite{DBLP:conf/aaai/Li00,DBLP:journals/tsmc/Brafman04,DBLP:journals/amai/Gelder05} Given that $x\up y$ and $\olnot{x}\up \olnot{y}$, equivalent literal substitution substitutes $x$ for $y$.
\item \textbf{Extension to Failed Literal Elimination}: given a variable $x$, if all clauses $C^R_{x}\in \{C\setminus \{x\}\mid x\in C\}$ have a literal $z\in C^R_{x}$ such that $x\up z$, the technique introduces unit clause $\{\olnot{x}\}$ and applies unit propagation rule to remove variable $x$.
\item \textbf{Extension to \TODO{``Implied Literals''?} and Equivalent Literals}: if, we do not have $x\up y$ but $x\up y$ would allow to apply \TODO{implied literal detection} or equivalent literal substitution, the technique checks if each clause $C^R_{\olnot{y}}=\{C\setminus\{\olnot{y}\}\mid \olnot{y}\in C\}$ contains a literal $z\in C^R_{\olnot{y}}$ such that $x\up z$.
If this is the case, we can introduce clause $x\lor \olnot{y}$ ($x\up y$ then follows) and then apply \TODO{implied literal detection}/equivalent literal substitution.
\item \textbf{TrimMaxSAT}~\cite{DBLP:conf/vmcai/PaxianRB21}. Given a set $S$ of literals, TrimMaxSAT-algorithm finds a subset $T\subseteq S$ of them such that for each $l\in T$, $F\ent \{\olnot{l}\}$. Given the set $T$ computed by TrimMaxSAT, we introduce unit clause $\{\olnot{l}\}$ for each $l\in T$ to the instance and apply unit propagation rule.
\end{itemize}

When the SAT-based techniques are lifted to MaxSAT, applying them will require an additional condition that the introduced change will not change the optimal cost of the intsance.
For example, we use a rule that bounded variable elimination or the extension to failed literal elimination are not applied to the objective literals.
Furthermore, in the context of MaxSAT, some of the techniques---in addition to introducing or removing clauses---may also change the objective function.
For example, if we have objective function $\obj \equiv 3\olnot{b}_1+\olnot{b}_2+1$, and unit clause $\{b_2\}$,
before applying unit propagation to remove variable $b_2$, we change the objective to $O\equiv 3\olnot{b}_1+1$.

The MaxSAT-specific preprocessing techniques which we consider in this work are the following.
\begin{itemize}
\item \textbf{(Group)-Subsumed Label Elimination}~\cite{DBLP:conf/ecai/BergSJ16,DBLP:conf/sat/KorhonenBSJ17}. Consider an objective literal $\olnot{b}$ with coefficient $c^{\olnot{b}}$ and a set of objective literals $L$ such that $\sum_{\olnot{b}_i\in L}c^{\olnot{b}_i}\le \olnot{b}$. Assume that $\{C\mid \olnot{b}\in C\}\subseteq \{C\mid \exists \olnot{b}_i\in L: \olnot{b}_i \in C\}$ and there does not exist a clause $C$ such that $b\notin C, \exists \olnot{b}_i\in L: b_i\in C$. Group-subsumed label elimination~\cite{DBLP:conf/sat/KorhonenBSJ17} fixes $b=1$, i.e., no cost for the objective literal $\olnot{b}$. Subsumed label elimination~\cite{DBLP:conf/ecai/BergSJ16} can be seen as a special case of group-subsumed label elimination with $|L|=1$.
\item \textbf{Intrinsic At-Most-Ones}~\cite{DBLP:journals/jsat/IgnatievMM19,IBJ22ClauseRedundancy}. Intrinsic at-most-ones detects sets of objective literals $L$ such that $\sum_{\olnot{b}\in l}\ge |L|-1$. For such a set $L$, new clause $\{b\mid \olnot{b}\in L\}\cup\{\olnot{b}^L\}$ (where $b^L$ is a fresh variable) is introduced and additionally, $\sum_{\olnot{b}\in L} -w^L\olnot{b}+w^L\olnot{b}^L+|L-1|w^L$ is added to the objective, where $w^L=\min (\{c^{\olnot{b}}\mid \olnot{b}\in L\})$ (but it is also possible to use some other value for $w^L$).
\item \textbf{Binary Core Removal}~\cite{DBLP:conf/focs/Gimpel64,DBLP:conf/sat/KorhonenBSJ17}. Assume the following three things: (i) $F$ contains a clause $\{\olnot{b}_C, \olnot{b}_D\}$ for two objective literals $\olnot{b}_C$ and $\olnot{b}_D$, (ii) $\olnot{b}_C$ and $\olnot{b}_D$ have the same coefficient $w$ in $O$, and (iii) the negations $b_C$ and $b_D$ do not appear in any clauses of $F$.
Assume additionally that $\olnot{b}_C$ and $\olnot{b}_D$ do not appear together in other clauses than in the core $\{\olnot{b}_C, \olnot{b}_D\}$ and that both appear in at least one other clause of $F$.
Binary core removal replaces all clauses where $\olnot{b}_C$ or $\olnot{b}_D$ appear with non-tautological clauses in $\{ C\cup D\cup \{\olnot{b}_{CD}\}\setminus\{\olnot{b}_C, \olnot{b}_D\}  \mid \olnot{b}_C\in C, \olnot{b}_D\in D\}$, where $\olnot{b}_{CD}$ is a fresh variable. Additionally, the objective function is modified by adding $-w \olnot{b}_C -w \olnot{b}_D +w\olnot{b}_{CD}+w$.
\item \textbf{Label Matching}~\cite{DBLP:conf/sat/KorhonenBSJ17}. Assume that (i) $\formula$ contains clauses $C\lor \olnot{b}_C$ and $D\lor \olnot{b}_D$ (ii) $\olnot{b}_C$ and $\olnot{b}_D$ are objective literals with the same coefficient in $\obj$, (iii) Variables $b_C$ and $b_D$ do not appear (in either polarity) in other clauses of $\formula$, (iv) $C\lor D$ is a tautology. Label matching replaces $b_C$ and $b_D$ with a fresh variable $b_{CD}$ (i.e., remove clauses $C\lor \olnot{b}_C$ and $D\lor \olnot{b}_D$, introduce $C\lor \olnot{b}_{CD}$, $D\lor \olnot{b}_{CD}$ instead) and adds $-w\olnot{b}_C-w\olnot{b}_D+w\olnot{b}_CD$ to the objective function.
\item \textbf{Hardening}~\cite{DBLP:conf/sat/MorgadoHM12,DBLP:conf/cp/AnsoteguiBGL12,IBJ22ClauseRedundancy}: given a solution $\tau$ with cost $\obj(\tau)=W$, each objective literal $\olnot{b}$ with $c^{\olnot{b}}>W$ can be fixed to $b=1$ (i.e., introduce a unit clause $\{b\}$ and then apply the unit propagation rule to remove variable $b$).
\end{itemize}



\paragraph{SAT-based Techniques.}
Given that we know how to log a proof for a preprocessing technique in SAT, logging the proof for a MaxSAT-lifting of the technique is relatively straightforward.
The
Whenever we eliminate a variable that is in the objective function, we need to update the objective function.

Since we use bounded variable elimination as a step in the proof for binary core removal, we give here the proof for bounded variable elimination as a concrete example of proofs for SAT-based techniques.
Assume we are using bounded variable elimination to eliminate variable $x$.
As a precondition for bounded variable elimination in MaxSAT setting, we assume that $x$ is not an objetive variable (i.e., neither $x$ nor $\olnot{x}$ appear in the objective function).
Bounded variable elimination introduces nontautological clauses in set $\mathcal{C}_{x}\otimes \mathcal{D}_{\olnot{x}} = \{C_x\otimes D_{\olnot{x}}\mid C\in \mathcal{C}_{x}, D_{\olnot{x}}\in \mathcal{D}_{\olnot{x}}\}$ of clauses and remove clauses in $\mathcal{C}_{x}$ and $\mathcal{D}_{\olnot{x}}$.

Let $C_i\otimes D_j$ be one of the clauses we are going to introduce.
We introduce $C_i\otimes D_j$ as a sum of constraints $C_i$ and $D_j$, which indeed yields $C_i\otimes D_j$.
After all nontautological clauses in $\mathcal{C}_{x}\otimes \mathcal{D}_{\olnot{x}}$ are introduced in this manner, the next step is to remove the clauses in $\mathcal{C}_{x}$ and $\mathcal{D}_{\olnot{x}}$.
We begin by logging a proof for removing each clause in $\mathcal{C}_{x}$ with witness $x\rightarrow 1$.
Assume we are removing clause $C_i\in \mathcal{C}_{x}$.
For the proof to be correct with witness $x\rightarrow 1$, we need to be able to prove for each clause $D_j\in \mathcal{D}_{\olnot{x}}$ that clause $D_j\setminus \{\olnot{x}\}$ is logically entailed
by the formula when each literal $C_i\setminus\{x\}$ is assigned to $0$.
This indeed follows by standard RUP check: when we set each $l_1\in C_i\setminus\{x\}$ and $l_2\in D_j\setminus\{\olnot{x}\}$ to false, this falsifies clause $C_i\otimes D_j$, which we have introduced into the formula.
(If $C_i\otimes D_j$ was a tautology and thus not introduced in the formula, there is some $l_1\in C_i\setminus\{x\}$ for which $\olnot{l}_1\in D_j\setminus\{\olnot{x}\}$, which, again, implies we have a contradiction.)
Thus each removal of $C_i$ is correct, and \veripb is able to autoprove each removal of clause $C_i$.

Finally, we remove each clause $D_j\in  \mathcal{D}_{\olnot{x}}$ with $x\rightarrow 0$ as a witness.
Since at this point all clauses where $x$ appeared have already bean removed, each of these steps is trivial.


\paragraph{Group-Subsumed Label Elimination.}
Assume that the preconditions for applying group-subsumed label elmination hold: (i) there is an objective literal $\olnot{b}$ with coefficient $c^{\olnot{b}}$ and a set of objective literals $L$ such that $\sum_{\olnot{b}_i\in L}c^{\olnot{b}_i}\le \olnot{b}$, (ii)  $\{C\mid \olnot{b}\in C\}\subseteq \{C\mid \exists \olnot{b}_i\in L: \olnot{b}_i \in C\}$, and (iii) there does not exist a clause $C$ such that $b\notin C, \exists \olnot{b}_i\in L: b_i\in C$.

The first step to log a proof is to introduce constraint $b\ge 1$
with witness $b_i\rightarrow 0$ for all $\olnot{b}_i\in L$, $b\rightarrow 1$.
Notice first, that the witness satisfies the new constraint, and has at least as good objective value as falsifying the new constraint.
Consider now the constraints of the instance that are affected by the witness.
The precondition (ii) guarantees that each clause $C$ with $\olnot{b}\in C$ is satisfied by the witness.
Finally, the precondition (iii) guarantees that each clause $C$ with $b_i\in C$ for some $\olnot{b}_i\in L$ is satisfied by the witness.

The rest of the proof is trivial. The objective function is updated and the simplifications that follow from fixing $b=1$ are applied.

\paragraph{Intrinsic At-Most-Ones.}
Proof logging for intrinsic at-most-ones has been previously studied in~\cite{BBNOV23CertifiedCoreGuided}.

\paragraph{Binary Core Removal.}
Assume that the preconditions for binary core removal hold: (i) $F$ contains a clause $\{\olnot{b}_C, \olnot{b}_D\}$ for two objective literals $\olnot{b}_C$ and $\olnot{b}_D$, (ii) $\olnot{b}_C$ and $\olnot{b}_D$ have the same coefficient $w$ in $O$, (iii) the negations $b_C$ and $b_D$ do not appear in any clauses of $F$, and (iv) that $\olnot{b}_C$ and $\olnot{b}_D$ do not appear together in other clauses than in the core $\{\olnot{b}_C, \olnot{b}_D\}$ and that both appear in at least one other clause of $F$.

The first step of our proof for binary core removal is to apply at-most-ones with $\{\olnot{b}_C, \olnot{b}_D\}$ as the set $L$.
This updates the objective function so that $-w\olnot{b}_C-w\olnot{b}_D+w\olnot{b}_{CD}+w$ is added, and the clause $\{b_C, b_D, \olnot{b}_{CD}\}$ is introduced to the instance as a new clause.
Notice that after updating the objective function, $b_C$ and $b_D$ are no longer objective variables, which enables to use bounded variable elimination on them.

The second step is to apply bounded variable elimination on variable $b_C$.
Literal $\olnot{b}_C$ appears in clauses $\{\olnot{b}_C, \olnot{b}_D\}$ and a set of clauses $C_i\lor \olnot{b}_C$.
Literal $b_C$ appears only in then clause $\{b_C, b_D, \olnot{b}_{CD}\}$ (the clause introduced during the at-most-ones step).
Bounded variable elimination on $b_C$ yields a set of clauses
$C_i\lor b_D \lor \olnot{b}_{CD}$. The original clauses are all removed.

The final step is to apply bounded variable elimination on variable $b_D$.
The literal $b_D$ appears in clauses $C_i\lor b_D \lor \olnot{b}_{CD}$ and the literal $\olnot{b}_D$ in clauses $D_i\lor \olnot{b}_D$.
Bounded variable elimination on $b_D$ thus yields clauses $C_i\lor D_i\lor \olnot{b}_{CD}$.


\paragraph{Label Matching.}
Assume that the preconditions for label matching hold: (i) $\formula$ contains clauses $C\lor \olnot{b}_C$ and $D\lor \olnot{b}_D$ (ii) $\olnot{b}_C$ and $\olnot{b}_D$ are objective literals with the same coefficient $w$ in $\obj$, (iii) Variables $b_C$ and $b_D$ do not appear in other clauses of $\formula$, (iv) $C\lor D$ is a tautology.
As $C\lor D$ is tautology, w.l.o.g. assume $x\in C$, $\olnot{x}\in D$.

First, we introduce clause $\{b_C, b_D\}$ with witness $b_C\rightarrow \olnot{x}, b_D\rightarrow x$.
Indeed, every optimal solution sets either $b_C=0$ or $b_D=0$.

The next step is to introduce a new variable $b_{CD}$, with encoding $\olnot{b}_{CD} = \olnot{b}_C + \olnot{b}_D$.
The clause $\{b_C, b_D\}$ introduced first makes possible that the equality holds even though the variables are binary.

Then, we update the objective function by adding $-w\olnot{b}_C-w\olnot{b}_D+w\olnot{b}_{CD}$.
The encoding of $b_{CD}$ makes this step correct.
Next step is to introduce clauses $C\lor \olnot{b}_{CD}$ and $D\lor \olnot{b}_{CD}$ to replace $C\lor \olnot{b}_C$ and $D\lor \olnot{b}_D$.
The new clauses are RUP; falsifying $C\lor \olnot{b}_{CD}$ will unit propagate $b_{CD}=0$ which means that the clause $C\lor \olnot{b}_C$ is falsified (and similarly for $D\lor \olnot{b}_{CD}$).
To delete $C\lor \olnot{b}_C$ and $D\lor \olnot{b}_D$ we use witness $\{b_C\rightarrow \olnot{x}, b_D\rightarrow x\}$.

Finally, we delete the constraints used to define $\olnot{b}_{CD} = \olnot{b}_C + \olnot{b}_D$ and clause $\{b_C, b_D\}$.


\paragraph{Hardening.}
Proof logging for hardening has also been previously studied in~\cite{BBNOV23CertifiedCoreGuided}.
In~\cite{BBNOV23CertifiedCoreGuided}, however, the hardening is done with the presence of so-called objective-improving constraints, i.e., $\obj\le UB-1$, where $UB$ is the cost of the best currently known solution.
In the context of preprocessing where the preprocessor should provide an equioptimal instance as an output, introducing objective-improving constraints to the instance is not possible.
To be able to do hardening, we need to take a different approach:
Given a solution $\tau$ with cost $\obj(\tau)=W$ and an objective literal $\olnot{b}$ with $c^{\olnot{b}}>W$,
we introduce unit clause $\{b\}$ with $\tau$ as the witness.

\fi

